Wilson Spaces, Snaith Constructions, and Elliptic Orientations

We construct a canonical family of even periodic $\mathbb{E}_{\infty}$-ring spectra, with exactly one member of the family for every prime $p$ and chromatic height $n$. At height $1$ our construction is due to Snaith, who built complex $K$-theory from $\mathbb{CP}^{\infty}$. At height $2$ we replace $\mathbb{CP}^{\infty}$ with a $p$-local retract of $\mathrm{BU} \langle 6 \rangle$, producing a new theory that orients elliptic, but not generic, height $2$ Morava $E$-theories. In general our construction exhibits a kind of redshift, whereby $\mathrm{BP}\langle n-1 \rangle$ is used to produce a height $n$ theory. A familiar sequence of Bocksteins, studied by Tamanoi, Ravenel, Wilson, and Yagita, relates the $K(n)$-localization of our height $n$ ring to work of Peterson and Westerland building $E_n^{hS\mathbb{G}^{\pm}}$ from $\mathrm{K}(\mathbb{Z},n+1)$.

==> ChromaticHeight.tex <==
Our goal in this section is to compute that the height of the ring $R_{h}$ is $h+1$.  We assume $h>0$ throughout. The same techniques could be used in the case that $h=0$ but we assume $p=0$ in various places so the formulas would be different. It is well known that $R_0=\KU_{(p)}$ is Landweber flat$.

Let $I_r$ be the $\BP_*$ ideal $I_r=(p, v_1,\ldots, v_{r-1})$ and let $I_{\infty}=(p,v_1,\ldots)$$.
\begin{thm$.
\label{height-of-R$.
$R_h$ is nonzero and the height of $R_h$ is $h+1$$.
\end{thm$.
To demonstrate that the height of $R_h$ is $h+1$, we show that in $\BP_*(R_h)/I_{h+1}$ the element $v_{h+1}$ is invertible. Let $u$ be the Hurewicz image of the bottom cell. Because $\BP_*(R_h)/I_{h+1} = u^{-1}\BP_*(\BPph)/I_{h+1}$, this reduces to a computation in $\BP_*(\BPph)/I_{h+1}$. We compute in \cref{x^p=vn*x} that $u^p = (-1)^huv_{h+1}$ in $\BP_*\BPph/I_{h+1}$ so $u^{p-1}-(-1)^hv_{h+1}\in \annu{h+1}$. Hence $v_{h+1}=(-1)^hu^{p-1}$ is invertible$.

 The element $u$ is given by $b_{(0)}^{\c p^{[h]}}$ in the Ravenel-Wilson basis.   It follows from the distributivity law for Hopf rings that $u^p = \left(b_{(0)}^{\c p^{[h]}}\right)^{*p} = [p]\circ b_{(1)}^{\c p^{[h]}}$ mod $p$.  To compute this, we start by showing (\Cref{vh*b1^p^h}) that in $Q\BP_*(\OSBPh{2*})/I_h$, one has for each $r$ the relation $[v_r]\circ b_{(1)}^{\c p^{r}}=-[v_{r+1}]\circ b_{(0)}^{\c p^{r+1}}\pmod{[I_r]},$ where $[I_{r}]$ denotes the ideal $([p], [v_1], \ldots, [v_{r-1}])$.  Then, using \Cref{Ih*b0^p^k=0}, we lift this to a statement before quotienting by $[I_r]$.  The relations for various $r$ link up to relate $[p]\c b_{(1)}^{\c p^{[h]}}$ to $v_{n+1}^{p-1} b_{(0)}^{\c p^{[h]}}$ mod $I_{h+1}$ and give a slightly more complicated formula mod $I_h$$.



\begin{lem$.
\label{bi^p^r$.
$.
%It isn't actually necessary to take indecomposables for this because I only consider the $p$-series through the range befor$.
% the first product occurs, but since $B(n)_*\OS{\BPn<r>}{2*}$ isn't a ring under $\circ$ I'm a little concerned about takin$.
% a quotient by a $\circ$ ideal without first taking indecomposables. The statement is good enough this way anyways$.
$.
Let $r<h$ be a nonnegative integer. In $Q\BP_*(\OSBPh{2*})/I_h$$.
\[[v_r]\c b_{(0)}^{\c p^r} \in [I_r]\$.
\end{lem$.
\begin{proof$.
The $p$-series of $\BP$ i$.
\[[p]_{\BP}(x) = O(x^{p^{h}}) \pmod{I_h}.\$.
The $p$-series of $\BPh$ i$.
\[[p]_{\BPh}(x) = v_rx^{p^r} + O(x^{p^{r+1}})\pmod{I_r}\$.
Thus, the Ravenel-Wilson relation $b([p]_{\BP}(x)) = [p]_{[\BPh]}(b(x))$ says in this case tha$.
\[O(x^{p^h}) = [v_r]\c \sum_{i} b_i^{\c p^{r}} x^{ip^{r}} + O(x^{p^{r+1}}) \pmod{[I_r], I_h}\$.
We extract the $x^{p^r}$ term from both sides. Since $r<h$, the coefficient of $x^{p^r}$ on the left hand side is $0$ and we deduce that $[v_r]\circ b_0^{\c p^r}=0\pmod{[I_r]}$$.
\end{proof$.


\begin{lem$.
\label{Ih*b0^p^k=0$.
    Let $r\leq h$ be a nonnegative integer and suppose $k\geq p^{[r-1]}$. If $x$ is an element of the augmentation ideal of $\BP_*\OSBPh{2k-2p^r+2}$ which maps to zero in $Q\BP_*(\OSBPh{2k-2p^r+2})/([I_{r}],I_h)$ then $x\c b_{(0)}^{\c k}=0$$.
\end{lem$.

\begin{proof$.
We work by induction on $r$. When $r=0$, the ideal $[I_r]$ is trivial and we need to check that $b_{(0)}\c x = 0$ if $x$ is decomposable. Say $x=a\s b$ where $a$ and $b$ are in positive degree. Since $\Delta(b_{(0)})=[0_2]\otimes b_{(0)} + [0_2]\otimes b_{(0)}$, distributivity says $b_{(0)}\c (a\s b) = ([0_2]\c a)\s (b_{(0)}\c b) + (b_{(0)}\c a) \s ([0_2] \c b) = 0$ since $y\c[0]=\eta(\epsilon(y))$ is the augmentation map$.

Now suppose $r>0$ and pick $x\in (\ker(\epsilon)^{\s 2}, [I_{r}])$. By induction we know that $(a\s b)\c b_{(0)}^{\c k}=0$ and $[v_i]\c b_{0}^{\c k}=0$ for $i<r-1$, so it suffices to show this for $x=[v_{r-1}]$.  We writ$.
\$.
[v_{r-1}]\c b_{(0)}^{\c k} =  \left([v_{r-1}]\c b_{(0)}^{\c p^{r-1}}\right) \c b_{(0)}^{\c (k - p^{r-1})}$.
\$.
By \Cref{bi^p^r}, $[v_{r-1}]\c b_{(0)}^{\c p^{r-1}}\in [I_{r-1}]$. Since $k-p^{r-1}\geq p^{[r-1]}-p^{r-1}=p^{[r-2]}$ the inductive hypothesis applies to show tha$.
\[\left([v_{r-1}]\c b_{(0)}^{\c p^{r-1}}\right) \c b_{(0)}^{\c (k - p^{r-1})}=0.\$.
\end{proof$.

\begin{lem$.
\label{vh*b1^p^h$.
Let $r \leq n$ be a nonnegative integer. In $Q\BP_*(\OSBPh{2})/([I_{r}],I_h)$$.
\[[v_r]\c b_{(1)}^{\c p^r} = \begin{cases$.
-[v_{r+1}]\c b_{(0)}^{\c p^{r+1}} & r < h-1\$.
-[v_{r+1}]\c b_{(0)}^{\c p^{r+1}}+v_{r+1} b_{(0)}  & r = h-1\$.
v_{r+1} b_{(0)}+v_{r}^pb_{(1)} & r = $.
\end{cases}\$.
\end{lem$.
\begin{proof$.
We hav$.
\[[p]_{\BP}(x) = \sumfgl{F}_{i=0}^{h+1} v_i x^{p^i} + O(x^{p^{h+2}}).\$.
Reducing modulo $I_{r}$ give$.
\[[p]_{\BP}(x) = v_rx^{p^{r}} +_{F} v_{r+1}x^{p^{r+1}} + O(x^{p^{r+2}})=v_rx^{p^{r}} + v_{r+1}x^{p^{r+1}} + O(x^{p^{r+2}}) \$.
Thus, in $Q\BP_*\OS{\BPn<h>}{2}/([I_{r}], I_h)$ the Ravenel-Wilson relation say$.
\[b(v_hx^{p^h} + v_{h+1}x^{p^{h+1}} + O(x^{p^{h+1}+1})) = [v_r]\c b(x)^{\c p^r} + [v_{r+1}]\c b(x)^{\c p^{r+1}}+ O(x^{p^{r+2}}).\$.
The $x^{p^{r+1}}$ coefficient on the right hand side is $[v_r]\c b_{(1)}^{\c p^r}+[v_{r+1}]\c b_{(0)}^{\c p^{r+1}}$$.
As long as $h>r+1$, the coefficient of $x^{p^{r+1}}$ in $b(v_{h}x^{p^{h}} + v_{h+1}x^{p^{h+1}})$ is $0$ an$.
\[0=[v_r]\c b_{(1)}^{\c p^r}+[v_{r+1}]\c b_{(0)}^{\c p^{r+1}}.\$.
If $h=r+1$ then the coefficient of $x^{p^{r+1}}$ in $b(v_{h}x^{p^{h}} + v_{h+1}x^{p^{h+1}})$ is $v_{r+1}b_{(0)}$ an$.
\[v_{r+1}b_{(0)}=[v_r]\c b_{(1)}^{\c p^r}+[v_{r+1}]\c b_{(0)}^{\c p^{r+1}}.\$.
If $h=r$ then the coefficient of $x^{p^{r+1}}$ in $b(v_{h}x^{p^{h}} + v_{h+1}x^{p^{h+1}})$ is $v_{h+1}b_{(0)}+v_{h}^pb_{(1)}$ an$.
\[v_{r+1}b_{(0)}+v_{r}^pb_{(1)}=[v_r]\c b_{(1)}^{\c p^r}\$.
where the $[v_{r+1}]$ term is missing because $r=h$ and $[v_{h+1}]=0$ in $\BP_*\BPph$$.
Isolating $[v_r]\c b_{(1)}^{\c p^r}$ in these equations gives the stated formula$.
\end{proof$.

\begin{lem$.
\label{x^p=vn*x-step$.
Let $r\leq h$. In $\BP_*(\OSBPh{2*})/I_h$$.
\[[v_r]\c b_{(0)}^{\c pp^{[r-1]}}\c b_{(1)}^{\c p^r} $.
\begin{cases$.
-[v_{r+1}]\c b_{(0)}^{\c pp^{[r]}} & r<h-1\$.
-[v_{r+1}]\c b_{(0)}^{\c pp^{[r]}} + v_{h}b_{(0)}^{\c p^{[r]}} & r=h-1\$.
-v_{h+1} b_{(0)}^{\c p^{[h]}} + v_{h}^pb_{(0)}^{\c pp^{[h-1]}}\c b_{(1)} & r=h\$.
\end{cases}\$.
\end{lem$.
\begin{proof$.
Combine \Cref{vh*b1^p^h} and \Cref{Ih*b0^p^k=0}$.
\end{proof$.


\begin{prop$.
\label{x^p=vn*x$.
Let $h$ be a nonnegative integer. Then in $\BP_*(\OS{\BPn<h>}{2p^{[h]}})/I_h$$.
\$.
    \left(b_{(0)}^{\c p^{[h]}}\right)^{\s p$.
    =(-1)^{h}\left$.
        v_{h+1}b_{(0)}^{\c p^{[h]}$.
        + v_h^pb_{(0)}^{\c pp^{[h-1]}}\c b_{(1)$.
        - v_hb_{(0)}^{\c p^{[h-1]}}\c b_{(1)}^{\c p^h$.
    \right)$.
\$.
\end{prop$.
\begin{proof$.
\Cref{x^p=vn*x-step} gives the following chain of equalities$.
\begin{align*$.
    (b_{(0)}^{\c p^{[h]}})^{\s p$.
    &= [p]\c b_{(1)}^{\c p^{[h]}}\$.
    &=  -[v_1]\c b_{(0)}^{\c p} \c b_{(1)}^{\c (p^{[h]}-1)} \$.
    &=  +[v_2]\c b_{(0)}^{\c pp^{[1]}}\c b_{(1)}^{\c (p^{[h]}-p^{[1]})}\$.
    &\vdotswithin{=}\\[-3pt$.
    &= \pm[v_{h-1}]\c b_{(0)}^{\c pp^{[h-2]}} \c b_{(1)}^{\c (p^h+p^{h-1})}\$.
    &= \mp[v_{h}]\c b_{(0)}^{\c pp^{[h-1]}} \c b_{(1)}^{\c p^h} \pm v_hb_{(0)}^{\c p^{[h-1]}}\c b_{(1)}^{\c p^h}\$.
    &=\mp v_{h+1}b_{(0)}^{\c p^{[h]}} \mp v_h^pb_{(0)}^{\c pp^{[h-1]}}\c b_{(1)} \pm v_hb_{(0)}^{\c p^{[h-1]}}\c b_{(1)}^{\c p^h}\$.
\end{align*$.
\end{proof$.

\begin{cor$.
In $\BP_*(R_{h})/I_{h+1}$, $(b_{(0)}^{\c p^{[h]}})^{p-1} = (-1)^hv_{h+1}$ and $v_{h+1}$ is invertible. Also, $\BP_*(R_{h})/I_{h+2}=0$ and so $L_{K(h+2)}R_{h}=0$$.
\end{cor$.



==> ModpWilson.tex <==
For $k\leq \ph$ there is a surjection $E_*\OS{BP}{*}\to E_*\OS{\BPh}{*}$. The kernel of this map is the Hopf ring ideal $([v_{h+1}], \ldots, )$. Thus, for $*\leq 2\ph$, $E_*\OS{\BPh}{*} \cong E_*\OS{BP}{*}/([v_{h+1}],\ldots )$ so \Cref{ravenel-wilson-main} tells us the complex oriented cohomology of all Wilson spaces$.

\begin{thm}[{\cite[4.18(ii)]{Ravenel-Wilson}}$.
$\HFp_*\OS{BP}{*}$ is a polynomial algebra$.
\end{thm$.

Ravenel and Wilson give a basis for $QH_*\OS{BP}{*}$. We will use this to get a basis for $QH_*\OS{BPh}{2k}$ for $k<p^{[h]}$ and a spanning set when $k=p^{[h]}$. First we recall the Ravenel-Wilson basis. Define elements in $H_*\OS{\BP}{*}$.
\[[v^I]b^J=[p^{i_0}v_1^{i_1}v_2^{i_2}\cdots]\circ b_{j_0}^{\circ j_0}\circ b_{(1)}^{\circ j_1}\$.
where $I=(i_1,\ldots)$ and $J=(j_0,j_1,\ldots)$ are sequences of nonnegative integers almost all $0$. Let $\Delta_k$ be the sequence with $1$ in the $k$h place and zeroes elsewhere$.

\begin{dfn}[{\cite[Definition 5.2]{Ravenel-Wilson}}$.
Let $e(J)$ be the maximum $n$ such that it is possible to write $J=p\Delta_{k_1}+\cdots + p^n\Delta_{k_n}+J'$ where $k_1\leq\cdots\leq k_n$ and $J'$ is nonnegative. Call $[v^I]b^J$ \emph{allowable} if $i_n=0$ for $n\geq e(J)$$.
\end{dfn$.

\begin{thm}[{\cite[Theorem 5.3(a)]{Ravenel-Wilson}}$.
The allowable $[v^I]b^J$ form a basis for $QH_*\OS{BP}{*}$$.
\end{thm$.

Let $S_{h,2k,*}$ be the polynomial ring on generators $[v^I]b^J$ with $I^{>h}=0$. There is  a surjection $f\colon H_*\OS{BP}{2k}\to S_{h,2k,*}$ given by quotienting out the ideal generated by allowable monomials $[v^I]b^J$ with $I^{>h}\neq 0$. There is a surjection $g\colon S_{h,2k,*}\to H_*\OS{\BPh}{2k}$ whose kernel is the ideal generated by the collection of not allowable monomials $f([v^I]b^J)$ with $I^{>h}\neq 0$$.

\begin{thm$.
When $k<\ph$, $S_{h,2k,*}\cong H_*\OS{\BPh}{2k}$$.
\end{thm$.


Given a sequence $I$, let $I^{\leq h}=(i_0,i_1,\ldots,i_h,0,\ldots)$ and $I^{>h} = (0,\ldots,0,i_{h+1},i_{h+2},\ldots)$$.
\begin{lem$.
Let $T\subseteq \HFp_*\OS{BP}{2k}$ be the additive subspace spanned by the nonallowable monomials $[v^I]b^J$ with $I^{>h}\neq 0$. The image $f(T)\subseteq S_{h,2k,*}$ is spanned by nonallowable monomials of the form $f([v_n]b^J)$ where $n>h$$.
\end{lem$.
In other words, $\ker(g)$ is the ideal generated by $f([v_n]b^J)$ where $n>h$ and $[v_n]b^J$ is not allowable$.

\begin{proof$.
Consider some nonallowable monomial $[v^I]\circ b^J$ with $I^{>h}\neq 0$. Let $i_n$ be the largest nonzero entry in $I$ and let $I'=I-\Delta_n$. If $I'=0$ there is nothing to show. Because $[v^I]\circ b^J$ is not allowable and $I'\neq 0$, neither is $[v^{I'}]\circ b^J$. We reduce this as a sum of allowable monomials $[v^{I'}]\circ b^J=\sum [v^{I_i}]b^{J_i}$. This means that $[v^I]\circ b^J=\sum [v_nv^{I_i}]b^{J_i}$. If $I_i\neq 0$ then $[v_nv^{I_i}]b^{J_i}$ is allowable and $f([v_nv^{I_i}]b^{J_i})=0$. Thus the relation we deduce i$.
\[f([v^I]\circ b^J)=\sum_{i|I_i=0} f([v_n]b^{J_i})\$.
So $f(T)$ is spanned by $f([v_n]b^{J_i})$ as desired$.
\end{proof$.

\begin{proof}[Proof of Theorem 6.6$.
We have shown that there is a surjection $g\colon S_{h,2k,*}\to H_*\OS{\BPh}{2k}$ with kernel generated by $f([v_n]b^{J_i})$ for $[v_n]b^{J_i}$ not admissible and $n>h$$.

The minimal $\circ$-weight of such a monomial is one of the form $[v_{h+1}]\circ b_{(i_1)}^{p}\circ \cdots\circ b_{(i_h)}^{(p^{h+1})}$. This has $\circ$ weight $-(p^{h+1}-1)+\sum_{i=1}^{h+1}p^i = pp^{[h]}-p^{h+1} + 1 = p^{[h]}$. It follows that for $k< p^{[h]}$, $\ker(g) = (0)$$.
\end{proof$.

\begin{thm$.
There is a filtration on $H_*\OS{\BPh}{2\ph}$ with associated graded polynomial tensor divided power. The indecomposibles whose $p$th powers vanish in the associated graded are those of the form $b_{(j_0)}\circ b_{(j_1)}^{\c p} \cdots \circ b_{(j_h)}^{\c p^h}$ with $j_0\leq \cdots\leq j_h$$.
\end{thm$.

We say that $[v^{I}]b^{J} < [v^{J'}]b^{J'}$ if$.
\begin{itemize$.
\item $|J| < |J'|$ o$.
\item $|J|=|J'|$ and $|[v^{I}]b^{J}| > |[v^{J'}]b^{J'}|$ o$.
\item $|J|=|J'|$ and $|[v^{I}]b^{J}| = |[v^{J'}]b^{J'}|$ and $J > J'$ in reverse lexicographic ordering$.
\end{itemize$.
Let $r_n$ be the coefficient of $s^{p^n}$ in $[p]_{[BP]}(s)$$.
\begin{thm}[{\cite[Lemma 4.15]{Ravenel-Wilson}}$.
The $r_n$ are defining relations for $H_*\OS{BP}{*}$. (What exactly do I want to say here? Need to make appropriate lifts of statements from the statements about indecomposibles.$...
\end{thm$.

We need the following mild refinement of \cite[Theorem 3.14]{Ravenel-Wilson}. Our proof is the same as the proof there$.
\begin{lem$.
\label{strengthened-3.14$.
\begin{align*$.
r_n &= \sum_{i=0}^n[v_i]b_{(n-i)}^{\c p^i} \pmod{[I]^{\c 2}, [I]^{\s 2}$.
\tag{a}\$.
r_n &= \sum_{i=1}^n[v_i]b_{(n-i)}^{\c p^i} \pmod{[I]^{\c 2}, \ker(\epsilon)^{\s p}}\tag{b$.
\end{align*$.
\end{lem$.

\begin{proof$.
Because $[p]_{BP}(s) = \sum_{n\geq 0}v_ns^{p^n} \pmod{I^2}$, it follows tha$.
\begin{align*$.
[p]_{BP}(s$.
&= \bigast_{n\geq 0} [v_n]\circ b(s)^{\circ p^n}\pmod{[I]^{\c 2}}\$.
&= \sum_{\geq 0}[v_n]\circ b(s)^{\circ p^n} \pmod{[I]^{\c 2}, [I]^{\s 2}$.
\end{align*$.
so this proves (a)$.
To check (b), note that $b(s)=\sum b_{(i)}s^{p^i} \pmod{[I]}$, so the extra terms that show up correspond to ways of writing $p^n = \sum_{i=1}^k p^{a_i}$. There's one solution to this when $k=1$, which leads to the terms in our formula. The next smallest value of $k$ for which there is a solution is $k=p$$.
\end{proof$.

\begin{cor$.
\label{strengthened-5.3-alpha$.
For any $\circ$-monomial $[v^I]\circ b^J$ with $|I|=1$ there is an expression $[v^I]\circ b^J = \sum [v^{I_i}]\circ b^{J_i} + \sum [p]\circ b^{J_i}\pmod{[I]^{\circ 2},[I]^{\s 2}}$ where $[v^{I_i}]\circ b^{J_i}$ is admissible and $|I_i|=1$$.
\end{cor$.

\begin{proof$.
Analyze the algorithm given in the proof of \cite[Theorem 5.3(a)]{Ravenel-Wilson} using \Cref{strengthened-3.14}(a) in place of \cite[Theorem 3.14]{Ravenel-Wilson}$.
\end{proof$.


\begin{lem$.
\label{strengthened-5.3$.
If $x=[v^I]\circ b^J$ is a $\circ$-monomial with $I>0$ and $x\in [I]^{\circ n}$ the$.
\[x=\sum [v^{I_i}]\circ b^{J_i} +\sum [p]\circ [v^{I_i'}]\circ b^{J_i'} \pmod{I^{\circ n+1},\left([I]^{\circ n}\right)^{\s 2}, \ker(\epsilon)^{p^2}}\$.
where $|I_i|=n$, $|I_i'| = n-1$ and $[v^{I_i}]\circ b^{J_i}$ is admissible for all $i$$.
\end{lem$.

\begin{proof$.
By induction on $n$. When $n=1$, this is \Cref{strengthened-5.3-alpha}. Suppose $x=[v_m]\circ [v^I]\circ b^J$ where $m$ is chosen as large as possible$.
Work by downwards induction on $m$. By induction on $n$, we can write $y=\sum [v^{I_i}]\circ b^{J_i} +\sum [p]\circ y'\pmod{[I]^{\circ n},\left([I]^{\circ (n-1)}\right)^{\s 2}}$ where $y'\in [I]^{\circ n-1}$. Now $[v_m]\circ [p]\circ y' \in \left([I]^{\circ n}\right)^{\s 2}$, $[v_m]\circ [I]^{\circ n+1}\subseteq [I]^{\circ n+2}$ and $[v_m]\circ \left([I]^{\circ (n)}\right)^{\s 2} \subseteq \left([I]^{\circ (n+1)}\right)^{\s 2}$$.
Our only concern is terms $[v_m]\circ[v^{I_i}]\circ b^{J_i}$ that are not admissible$.
Since $[v^{I_i}]\circ b^{J_i}$ is admissible, in order for this to happen we must have $[v^{I_i}] = [v_{m'}]\circ [v^{I_i'}]$ for $m'>m$. By downwards induction on $m$ these $\circ$-monomials also have a decomposition of the proper form$.
\end{proof$.

\begin{lem$.
\label{strengthened-5.3-*2$.
If $x\in \left([I]^{\circ n}\right)^{\s 2}$ the$.
\[x=\sum [v^{I_i}]\circ b^{J_i}\s z \pmod{\left([I]^{\circ n+1}\right)^{\s 2}, \ker(\epsilon)^{p+1}}\$.
where $|I_i|=n$ and $[v^{I_i}]\circ b^{J_i}$ is admissible for all $i$$.
\end{lem$.

\begin{proof$.
We can write $x=[p]^{[i]}\circ [v^I]\circ b^J \s z$ where $[v^I]\circ b^J$ is a $\circ$ monomial with $|I|=n-i$ and $z\in\ker(\epsilon)$. If $i\geq 1$ then $x\in \ker(\epsilon)^{p+1}$ and so $x=0\pmod{\left([I]^{\circ n+1}\right)^{\s 2}, \ker(\epsilon)^{p+1}}$ is an equation of the desired form. If $i=0$, we apply \Cref{strengthened-5.3} to write$.
\end{proof$.

\begin{lem$.
\label{tN<adm-in-[I]$.
Suppose $[v^I]\circ b^J$ is an admissible monomial of degree $|t_N|$ and $I>0$. Then $t_N < [v^I]\circ b^J \s z$$.
\end{lem$.

\begin{proof$.
Case (1) in the definition of $<$ applies$.
\end{proof$.

\begin{lem$.
\label{tN<ker(e)^p+1$.
If $|x| = |t_N|$ and $x\in \ker(\epsilon)^{\s (p+1)}$ then $t_N<x$$.
\end{lem$.

\begin{proof$.
Since $t_N$ has minimal $\circ$ weight, it's impossible that $x<t_N$ because of case (1). Since $x$ is $\s$-decomposable into $p+1$ parts, one of those parts must have degree less than $|t_N|/p$. On the other hand, $t_N$ is only decomposable into $p$ parts, each of which has degree $|t_N|/p$. Thus, case (2) applies and $t_N < x$$.
\end{proof$.


\begin{lem$.
\label{tN<p^2x$.
Suppose $|x|=|t_N|$. Then $t_N < [p^2]\circ x$$.
\end{lem$.

\begin{proof$.
$[p^2]\circ x \in \ker(\epsilon)^{\s p^2}$ so \Cref{tN<ker(e)^p+1} applies$.
\end{proof$.

\begin{lem$.
\label{tN<[p]I$.
Suppose $x\in [I]$ and $|x|=|t_N|$. Then $t_N<[p]\circ x$$.
\end{lem$.

\begin{proof$.
We show this for $x\in [I]^{\circ n}$ for $n\geq 1$ by downwards induction on $n$. For $n$ large enough $[I]^{\circ n}$ contains only $0$ in degree $|t_N|$$.

Suppose $x\in [I]^{\circ n}$ is a $\s$-monomial, say $x=[v^{I}]\circ b^J \s x'$ for $|I|\geq n$. By \Cref{strengthened-5.3}$.
\[x=\sum [v^{I_i}]\circ b^{J_i}\s x' + [p]\circ x''\pmod{[I]^{\circ (n+1)}, \left([I]^{\circ n}\right)^{\s2},\ker(\epsilon)^{p+1}}\$.
where $|I_i|\geq n >0$ for all $i$$.
Thus$.
\[[p]\circ x = \sum [p]\circ[v^{I_i}]\circ b^{J_i}\s t_i + [p^2]\circ x'' + [p]\circ y + [p]\circ z\$.
where $y\in[I]^{\circ (n+1)}$ and $z\in \left([I]^{\circ n}\right)^{\s2}$$.
By our inductive hypothesis, $t_N<[p]\circ y$. By \Cref{tN<ker(e)^p+1}, $t_N<[p]\circ z$ and $t_N<[p^2]\circ x''$. Either $[p]\circ[v^{I_i}]\circ b^{J_i}=([v^{I_i}]\circ b^{J_i'})^{*p}$ for $[v^{I_i}]\circ b^{J_i'}$ admissible or $[p]\circ[v^{I_i}]\circ b^{J_i}=0$$.
In the first case, \Cref{tN<adm-in-[I]} says that $t_N < [p]\circ[v^{I_i}]\circ b^{J_i}$ and in the second case this is immediate$.
\end{proof$.

\begin{lem$.
Suppose $m$ and $n$ are positive integers, one of which is at least $2$. If $x\in \left([I]^{\c m}\right)^{\s n}$ then $t_N<x$$.
\end{lem$.

\begin{proof$.
Fix $t_N$ and work by downwards induction on $m+n$. If $m+n$ is large enough, $\left([I]^{\c m}\right)^{\s n}$ is $0$ in the appropriate bidegree$.
\end{proof$.
This unpacks into the following two lemmas$.
\begin{lem$.
Suppose $x\in [I]^{\s 2}$ and $|x|=|t_N|$. Then $t_N<x$$.
\end{lem$.

\begin{lem$.
Suppose $x\in [I]^{\circ 2}$ and $|x|=|t_N|$. Then $t_N<x$$.
\end{lem$.

\begin{proof$.
We show this is true for $x\in I^{\circ i}$ by downwards induction on $i$. In a fixed degree, for $i$ large enough, $[I]^{\circ i}$ only contains $0$ and $t_N<0$. Suppose the statement is true for $i+1 > 2$, we show it is true for $i$$.


It suffices to check this for $\s$-monomials. It's possible to write $x = [p^j]\circ y \s z$ for $y\in [I]^{\circ i-j}$ a $\circ$ monomial and $z$ a $\s$-monomial. If $j>1$ then $x\in \ker(\epsilon)^{p}$ so $t_N<x$. If $j=1$ then either $z\in\ker(\epsilon)$ and $x\in \ker(\epsilon)^{p+1}$ so $t_N<x$ by \Cref{tN<ker(e)^p+1} or by $\Cref{strengthened-5.3}$, $x= \sum [p]\circ[v^{I_i}]\circ b^{J_i}\pmod{\left([I]^{\circ i-j}\right)^{\s 2},\ker(\epsilon)^{p+1}}$ for $|I_i|=i-j-1$$.

Apply \Cref{strengthened-5.3} to write $y = \sum [v^{I_i}]\circ b^{J_i}+[p]\circ y+\sum [v^{I_i}]\circ b^{J_i}$ where $y_1\in [I]^{\circ i-j+1}$, $y_2\in $  $y_3\in \ker(\epsilon)^{p}$$.
\end{proof$.


\begin{lem$.
$r_N = s_N^{*p} + \text{terms in higher filtration}$.
\end{lem$.


\begin{proof$.

\end{proof}$.
